CTRQNets & LQNets: Continuous Time Recurrent and Liquid Quantum Neural Networks

Neural networks have continued to gain prevalence in the modern era for their ability to model complex data through pattern recognition and behavior remodeling. However, the static construction of traditional neural networks inhibits dynamic intelligence. This makes them inflexible to temporal changes in data and unfit to capture complex dependencies. With the advent of quantum technology, there has been significant progress in creating quantum algorithms. In recent years, researchers have developed quantum neural networks that leverage the capabilities of qubits to outperform classical networks. However, their current formulation exhibits a static construction limiting the system's dynamic intelligence. To address these weaknesses, we develop a Liquid Quantum Neural Network (LQNet) and a Continuous Time Recurrent Quantum Neural Network (CTRQNet). Both models demonstrate a significant improvement in accuracy compared to existing quantum neural networks (QNNs), achieving accuracy increases as high as 40\% on CIFAR 10 through binary classification. We propose LQNets and CTRQNets might shine a light on quantum machine learning's black box.

==> Background/DeepLearning.tex <==
Deep learning is the study of algorithms that bear a close relation to Neural Networks. Examples of this can be realized in applications such as \cite{chatgpt1,chatgpt2,ibm_cnn,NODES}. The scalability of these models is one of the key components for the media attention Deep Learning receives as they are only dependent on a set of parameters at a given time. It is also worthy to note that these models in essence are mathematical models which are optimized through various processes and in a sense bear no artificial intelligence in contrary to what is popular believed. The parameters which underlie these models are what the network "knows" and the patterns. These parameters may encode abstract patterns unknown from first glance as humans but due to the shear size of these parameters, it is impossible to know what these networks truly "know". This is what causes hesitation for real world applications of Machine Learning models as it is difficult to control these models\cite{ibm_explainable_ai,vox_unexplainable_chatgpt} and assess what they truly know and what they are capable of.However, through the use of new "liquid models"\cite{LNNS} it has been significantly clearer on how to control Deep Learning models and accurately assess them. The reasoning behind these models is the fact that we understand mathematics more than we understand Artificial Intelligence so if we can build a dynamic model which learns through means of time dependencies, it will be a easier task to assess the understanding of the model. Liquid Neural Networks only needed 19 Neurons to drive a car\cite{LNNS} where as traditional LSTMS need millions of Neurons \cite{LSTM} to perform this same task. These liquid models have a close representation of what is taken to be intelligence with the models being task aware and dynamic even after the training process is complete.

==> Background/MachineLearningIntro.tex <==
Machine learning is the study of developing intelligence through mathematical models. The field has been subject to increased media attention over the last 20 years due to the scalability of machine learning methods\cite{javapoint}.In fact, Machine Learning is a sub-field of Artificial Intelligence, with the latter being more well-known. By the name, Artificial Intelligence is concerned with developing artificial forms of intelligence, whether it be through biological processes (Synthetic Biological Intelligence)\cite{bio1,bio2,bio3,stanford_hai_biological_intelligence} or mathematical/computer processes, with the latter being known as Machine Learning. There is much to be said of the potential of either of the aforementioned methods, but due to the rich history of mathematics, there is a deeper understanding of how to further develop intelligence. Specifically, neural networks are of much interest due to the sheer amount of abstract patterns\cite{mitnn,ibmnn} they can learn, whereas other methods, such as Support Vector Machines, do not possess this property when dealing with large datasets \cite{svm1}. Both of these models pertain to a field known as Deep Learning, which originates from Neural Networks.

==> Background/QuantumML.tex <==
Quantum machine learning is a field with much research being done.
